Multi-Modal Multi-Instance Learning for Retinal Disease Recognition

This paper attacks an emerging challenge of multi-modal retinal disease recognition. Given a multi-modal case consisting of a color fundus photo (CFP) and an array of OCT B-scan images acquired during an eye examination, we aim to build a deep neural network that recognizes multiple vision-threatening diseases for the given case. As the diagnostic efficacy of CFP and OCT is disease-dependent, the network's ability of being both selective and interpretable is important. Moreover, as both data acquisition and manual labeling are extremely expensive in the medical domain, the network has to be relatively lightweight for learning from a limited set of labeled multi-modal samples. Prior art on retinal disease recognition focuses either on a single disease or on a single modality, leaving multi-modal fusion largely underexplored. We propose in this paper Multi-Modal Multi-Instance Learning (MM-MIL) for selectively fusing CFP and OCT modalities. Its lightweight architecture (as compared to current multi-head attention modules) makes it suited for learning from relatively small-sized datasets. For an effective use of MM-MIL, we propose to generate a pseudo sequence of CFPs by over sampling a given CFP. The benefits of this tactic include well balancing instances across modalities, increasing the resolution of the CFP input, and finding out regions of the CFP most relevant with respect to the final diagnosis. Extensive experiments on a real-world dataset consisting of 1,206 multi-modal cases from 1,193 eyes of 836 subjects demonstrate the viability of the proposed model.

==> backup.tex <==


\begin{figure}[thb!]
\centering
\subfigure[Multi-modal Input]{
\centering
\includegraphics[width=\columnwidth]{figures/fig1a.pdf}
% \caption{Multi-modal Input}
}
\subfigure[Heatmap on image]{
\centering
\includegraphics[width=\columnwidth]{figures/fig1b.pdf}
% \caption{Multi-modal Input}
}
% \vspace{-6mm}
\caption{\textbf{Overview of a case}} 
\label{fig:fig1a}
\end{figure}



%We denote $\mathbf{v}_c = \{v_{c,1}, \ldots, v_{c,n}\}$ and $\mathbf{v}_o = \{v_{o,1}, \ldots, v_{o,n}\}$ as the CFP and OCT's feature vectors extract from backbone. To handle the multi-modal input, we propose a multi-modal multi-instance learning network(MM-MIL). In this work MM-MIL consists of two parts, feature projection module and attention module. The feature projection module contains one linear projection, followed by layer normalization\cite{layer-norm}. For each modal, there is a corresponding feature projection module. Note that we share the parameters of projection module when stack multiple MM-MIL to reduce the training parameters. We use $\tilde{\mathbf{v}}_c  = \{\tilde{v}_{c,1}, \ldots, \tilde{v}_{c,n}\}$ and $\tilde{\mathbf{v}}_o  = \{\tilde{v}_{o,1}, \ldots, \tilde{v}_{o,n}\}$ to indicate the feature vector after projection. That is, 

%\begin{equation}
%\tilde{v}_{c,i} := LayerNorm(Linear_{2048 \times 2048}({v}_{c,i})),~~i=1,\ldots,n.
%\end{equation}

% \begin{equation}
% \tilde{v}_{o,i} := LayerNorm(Linear_{2048 \times 2048}({v}_{o,i})),~~i=1,\ldots,n),
% \end{equation}
%where $Linear$ indicates a fully connected layer. In the same manner, we can get $\tilde{\mathbf{v}}_o$.

%The two vectors are then concatenated into $\mathbf{v}_f  = %\{\tilde{v}_{c,1}, \ldots, \tilde{v}_{c,n}, \\
%\tilde{v}_{o,1}, \ldots, \tilde{v}_{o,n}\}$ as the input of %the attention module, which consists of two $Linear$ layers, where $tanh$ is its intermediate activation function and softmax ensures that the attention weights $\mathbf{a} = \{a_{1}, \ldots, a_{2n}\}$ sum to 1 \cite{icml18-mil}. Therefore, the attention weights $\mathbf{a}$ are obtained by

\begin{equation} \label{eq:ins-att}
\begin{split}
a_i := softmax(Linear_{128\times 1}(tanh (Linear_{2048 \times 128}(v_{f,i}))),\\
~~i=1,\ldots,2n.
\end{split}
\end{equation}

The output of attention module $\mathbf{a}$ represents the significance of different modalities and instances. For obtaining a final feature vector representation $\mathbf{v}$, attention-based feature aggregation is performed as a weighted sum of the instance features,

\begin{equation} \label{eq:feat-agg}
\mathbf{v} := \sum_{i=1}^{2n} a_i \cdot v_{f,i},
\end{equation}

The feature vector $\mathbf{v}$ then goes into the case-level classification layer. 


Our experiments show that a multi-modal input composed of one CFP and 12 OCT B-scans tends to incur the data imbalance problem, which means that the network relies too much on OCT information in the forward and backward process, causing the train process to converge to local minima. In order to tackle this problem, we propose a strategy of over sampling the CFP image to match the number of OCT b-scans. The 12 OCT scans of an examination are resized to $256\times256\times3$. And the CFP is resized to $512\times512\times3$. In the training phase, we use the OCT selected by the ophthalmologist plus the randomly selected OCT in a total number of 6. For CFP, 6 images are randomly cropped from the original image and then resized into $256\times256\times3$. As shown in Fig , in inference phase, for obtaining a fixed number of 12 CFPs, we resize the CFP into $256\times256\times3$, crop the four corners and the center of the raw CFP to get 6 images of size $256\times256\times3$. Then plus the horizontally flipped version of these. Thus, the input of CFP modal becomes $\mathbf{x}_c = \{x_{c,1}, \ldots, x_{c,n}\}$. The new version of network G is:

\begin{equation}\label{eq:basic}
\hat{y} := G(\mathbf{x}_c, \mathbf{x}_o),
\end{equation}



As shown in Fig, our proposed network consists of three blocks:  feature extraction backbone,  aggregation block multi-modal multi-instance learning network, which we term MM-MIL and case-level multi-label classification layer. The two modal inputs $\mathbf{x}_c$ and $\mathbf{x}_o$ are different in color, shape, etc. Like Wang \etal \cite{miccai19-amd}, we also use parallel backbones to extract features of different modalities. After making a trade-off between speed and performance, we use ImageNet pre-trained ResNet-50 \cite{cvpr2016-resnet} as our backbone. Consequently, each backbone results in an array of feature vectors of size $n\times2048$ respectively. The MM-MIL block receives feature vectors of different modalities, focuses on the significance of different modalities and instances, and finally outputs a case-level aggregated feature vector. The MM-MIL block can be easily stacked in multiple times in parallel. In the case of adding small parameters, the performance of the model can be significantly improved. Then, the feature vectors output by multiple MM-MILs are goes to the $Linear$ layer to obtain multi-label scores, and the mean pooling operation is used to obtain the average value of these scores. Finally, the sigmoid function is used to obtain the category probability scores $\hat{y}$.

We denote $y$ as the true label of the eye. And use binary cross entropy to calculate the loss between the probability $\hat{y}$ and $y$,

\begin{equation}\label{eq:basic}
loss := \frac{1}{m} \cdot \sum_{i=1}^{m} (y_i \cdot log(\hat{y}_i) + (1-y_i) \cdot log(1-\hat{y}_i)) ,
\end{equation}

In this sectio the wn, we describe the procedure for generating multi-modal activation maps. Attention weight $\mathbf{a}$ shows the significance of each feature vector. The feature vectors are obtained from the feature maps after spatial-wise global average pooling(SW-GAP). SW-GAP outputs the spatial average of the feature map. Therefore, the importance of each point on the feature vector is the importance of the corresponding feature map. We average the channel dimensions of each feature map as the activation map of the instance and then multiply the attention weight by the activation map to get the instance visualization.

To simplify the notation, we only show the calculation process of one instance. We define $\mathbf{f} = \{f_1, \ldots, f_{d}\}$ as one instance's feature maps with shape of $h\times w\times d$. Assuming there are h MM-MIL modules, we denotes $\mathbf{A} = \{A_1, \ldots, A_h\}$  as this instance's attention weight. Attention-based activation maps $M$ can be obtained as follows,
\begin{equation} \label{eq:visualize}
M := \frac{1}{h} \sum_{k=1}^{h} a_k \cdot \frac{1}{d} \cdot \sum_{i=1}^{d} F_i,
\end{equation}
To get the visualization of an examination, we need to map the CFP's parts back to the whole map. For the down-sampled activation map, it is up-sampled to the original size, and for the horizontal flip operation, the reverse flip is performed. Then combine the activation maps of CFP and OCT.


If normal is annotated, there is no symptom on both CFP and OCT images. The main symptom of ERM is the membranes on the inner surface of the retina, which is more obvious on OCT. The symptom of ME, accumulation of fluid in macular, is very clear in OCT, but is hard to distinguish from CFP. DR is mainly diagnosis by CFP. The occurrence of dryAMD is with geographic atrophy in CFP and irregular protrusion of retinal pigment epithelium in OCT. wetAMD is diagnosed in terms of choroidal neovascularization in OCT. We can observe PM by myopic crescent and spotty patchy lesion in CFP and choroidal atrophy in OCT.


The MM-CNN model~\cite{miccai19-amd} is the state-of-the-art in multi-modal fundus diagnosis. MM-CNN concatenates the feature of a CFP image and the feature of an OCT b-scan selected by the ophthalmologists to fuse multi-modal information. However, as shown in Fig. \ref{fig:radial-mode}, there are 12 b-scans produced in an only examination. Selecting the representative is reliable on ophthalmologists, which limits the application of the model and the diagnosis results depend on the quality of the manual selection. We compare different selection methods of MM-CNN, \eg \textit{first-frame}, \textit{middle-frame}, \textit{last-frame} and \textit{manual-frame}. As shown in Table \ref{tab:bscan-selection}, manual-frame model has a higher sensitivity, F1-score and AP than the other fixed-frame methods, proving that manual b-scan selection is necessary for MM-CNN.


  failed to converge.  due to  ConvNet is usually used in integrating multiple frames and fusing optical flow modal with RGB images in video recognition~\cite{cvpr17-twostream}. We try to compare MIL with 3D-ResNet~\cite{hara3dcnns} in OCT categorization. However, 3D-ResNet cannot converge on training set, which may be caused by numerous parameters of 3D networks and small dataset or 3D ConvNet is more suitable for raster data not radial data. Then, we use 3D-fused ResNet-50 which uses 2D-ResNet to extract features of OCT b-scans and then uses a 3D fusion module which consists of three 3D convolutions and a global average pooling. 3D-fused ResNet-50 get an AP of 0.7710, but it cannot give interpretation of that which b-scans matter.
  
  
  Instead of performing a single MM-MIL block, we can stack multiple MM-MIL blocks for diverse multi-modal representations. Vaswani \textit{et al.} propose to use multi-head self-attention (MHSA) in transformer to attend to information from different representation subspaces at different positions~\cite{nips2017-transformer}. We implement MM-MIL in similar style by stacking multiple MM-MIL blocks. For fundus diagnosis, different disease may focus on different instances, \eg DR usually focus on CFP image, while ME focus on OCT images. One instance weight is not enough when the two diseases exists simultaneously. 


==> tables/cfp-upsample.tex <==
\begin{table*}[]
    \caption[]{\textbf{CFP over sampling}}
    \label{tab:cfp-upsample}
    \resizebox{0.98\linewidth}{!}{
        \begin{tabular}{|lcccccccccccc|}
            \hline
            \multicolumn{1}{|l|}{\multirow{2}{*}{\textbf{CFP Inputs}}} & \multicolumn{5}{c|}{\textbf{Overall metrics}} & \multicolumn{7}{c|}{\textbf{AP of specific categories}} \\ \cline{2-13} 
            \multicolumn{1}{|l|}{} & \multicolumn{1}{c|}{\textit{AP}} & \multicolumn{1}{c|}{\textit{AUC}} & \multicolumn{1}{c|}{\textit{Sensitivity}} & \multicolumn{1}{c|}{\textit{Specificity}} & \multicolumn{1}{c|}{\textit{F1-score}} & \multicolumn{1}{c|}{\textit{Normal}} & \multicolumn{1}{c|}{\textit{ERM}} & \multicolumn{1}{c|}{\textit{ME}} & \multicolumn{1}{c|}{\textit{DR}} & \multicolumn{1}{c|}{\textit{dryAMD}} & \multicolumn{1}{c|}{\textit{wetAMD}} & \textit{PM} \\ \hline
            \textit{Single-modal} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
            \multicolumn{1}{|l|}{ResNet (CFP $\times$ 1)} & \multicolumn{1}{c|}{0.6827} & \multicolumn{1}{c|}{0.9025} & \multicolumn{1}{c|}{\textbf{0.6109}} & \multicolumn{1}{c|}{0.9500} & \multicolumn{1}{c|}{\textbf{0.7295}} & \multicolumn{1}{c|}{0.9830} & \multicolumn{1}{c|}{0.5508} & \multicolumn{1}{c|}{0.6405} & \multicolumn{1}{c|}{0.8738} & \multicolumn{1}{c|}{0.3879} & \multicolumn{1}{c|}{0.5277} & 0.8152 \\ \hline
            \multicolumn{1}{|l|}{MIL (CFP $\times$ 12)} & \multicolumn{1}{c|}{\textbf{0.7357}} & \multicolumn{1}{c|}{\textbf{0.9233}} & \multicolumn{1}{c|}{0.5969} & \multicolumn{1}{c|}{\textbf{0.9584}} & \multicolumn{1}{c|}{0.7244} & \multicolumn{1}{c|}{\textbf{0.9841}} & \multicolumn{1}{c|}{\textbf{0.6713}} & \multicolumn{1}{c|}{\textbf{0.6941}} & \multicolumn{1}{c|}{\textbf{0.9350}} & \multicolumn{1}{c|}{\textbf{0.4235}} & \multicolumn{1}{c|}{\textbf{0.5747}} & \textbf{0.8674} \\ \hline
            \textit{Multi-modal} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l}{} & \multicolumn{1}{l|}{} \\ \hline
            \multicolumn{1}{|l|}{MM-MIL (CFP $\times$ 1)} & \multicolumn{1}{c|}{0.7872} & \multicolumn{1}{c|}{\textbf{0.9286}} & \multicolumn{1}{c|}{0.6729} & \multicolumn{1}{c|}{0.9468} & \multicolumn{1}{c|}{0.7640} & \multicolumn{1}{c|}{0.9789} & \multicolumn{1}{c|}{\textbf{0.7753}} & \multicolumn{1}{c|}{\textbf{0.855}} & \multicolumn{1}{c|}{0.7766} & \multicolumn{1}{c|}{0.4337} & \multicolumn{1}{c|}{0.8235} & 0.8675 \\ \hline
            \multicolumn{1}{|l|}{MM-MIL (CFP $\times$ 12)} & \multicolumn{1}{c|}{\textbf{0.8097}} & \multicolumn{1}{c|}{0.9261} & \multicolumn{1}{c|}{\textbf{0.7311}} & \multicolumn{1}{c|}{\textbf{0.9635}} & \multicolumn{1}{c|}{\textbf{0.8214}} & \multicolumn{1}{c|}{\textbf{0.9888}} & \multicolumn{1}{c|}{0.7576} & \multicolumn{1}{c|}{0.7802} & \multicolumn{1}{c|}{\textbf{0.8617}} & \multicolumn{1}{c|}{\textbf{0.5326}} & \multicolumn{1}{c|}{\textbf{0.8325}} & \textbf{0.9149} \\ \hline
            \end{tabular}
    }
\end{table*}

==> tables/conv3d.tex <==
\begin{table}[]
    \caption{Performance of MIL and Conv3D on OCT single-modal recognition. MIL has similar AUC with Conv3D, but have better AP, sensitivity, specificity and F1-score. MIL has better performance than Conv3D in processing multiple instance recognition task.}
    \label{tab:conv3d}
    \resizebox{\linewidth}{!}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline
\textbf{Model} & \textbf{AP} & \textbf{AUC} & \textbf{Sen.} & \textbf{Spe.} & \textbf{F1} \\ \hline
Conv3D (OCT) & 0.771 & \textbf{0.9283} & 0.6324 & 0.937 & 0.7141 \\ \hline
MIL (OCT) & \textbf{0.7748} & 0.9281 & \textbf{0.664} & \textbf{0.9495} & \textbf{0.7417} \\ \hline
\end{tabular}
}
\end{table}

==> tables/num-mm-mil.tex <==
\begin{table*}[]
    \caption{\textbf{Performance of MM-MIL with varied number of heads}.}
    \label{tab:num-mm-mil}
    \resizebox{\linewidth}{!}{
        \begin{tabular}{|l|c|c|c|c|c|c|c|c|c|c|c|c|}
            \hline
            \multirow{2}{*}{\textbf{\#Heads}} & \multicolumn{5}{c|}{\textbf{Overall performance}} & \multicolumn{7}{c|}{\textbf{AP per category}} \\ \cline{2-13} 
             & \textit{AP} & \textit{AUC} & \textit{Sen.} & \textit{Spe.} & \textit{F1-score} & \textit{Normal} & \textit{ERM} & \textit{ME} & \textit{DR} & \textit{dryAMD} & \textit{wetAMD} & \textit{PM} \\ \hline
            MM-MIL$\times$ 1 & 0.8097 & 0.9261 & 0.7311 & 0.9635 & 0.8214 & 0.9888 & 0.7576 & 0.7802 & 0.8617 & 0.5326 & 0.8325 & \textbf{0.9149} \\ \hline
            MM-MIL$\times$ 2 & 0.8348 & 0.9424 & \textbf{0.7577} & 0.9664 & \textbf{0.8393} & 0.9933 & 0.7628 & 0.8409 & 0.8898 & 0.5584 & 0.8969 & 0.9014 \\ \hline
            MM-MIL$\times$ 4 & \textbf{0.8539} & \textbf{0.9545} & 0.7431 & 0.9643 & 0.8291 & \textbf{0.9940} & 0.7793 & \textbf{0.9038} & 0.8939 & \textbf{0.6220} & 0.9035 & 0.8808 \\ \hline
            MM-MIL$\times$ 8 & 0.8534 & 0.9505 & 0.7335 & \textbf{0.9720} & 0.8285 & 0.9922 & \textbf{0.7939} & 0.8633 & \textbf{0.9165} & 0.5969 & \textbf{0.9105} & 0.9006 \\ \hline
            \end{tabular}
    }
\end{table*}
